Max-Sliced Mutual Information

Quantifying the dependence between high-dimensional random variables is central to statistical learning and inference. Two classical methods are canonical correlation analysis (CCA), which identifies maximally correlated projected versions of the original variables, and Shannon's mutual information, which is a universal dependence measure that also captures high-order dependencies. However, CCA only accounts for linear dependence, which may be insufficient for certain applications, while mutual information is often infeasible to compute/estimate in high dimensions. This work proposes a middle ground in the form of a scalable information-theoretic generalization of CCA, termed max-sliced mutual information (mSMI). mSMI equals the maximal mutual information between low-dimensional projections of the high-dimensional variables, which reduces back to CCA in the Gaussian case. It enjoys the best of both worlds: capturing intricate dependencies in the data while being amenable to fast computation and scalable estimation from samples. We show that mSMI retains favorable structural properties of Shannon's mutual information, like variational forms and identification of independence. We then study statistical estimation of mSMI, propose an efficiently computable neural estimator, and couple it with formal non-asymptotic error bounds. We present experiments that demonstrate the utility of mSMI for several tasks, encompassing independence testing, multi-view representation learning, algorithmic fairness, and generative modeling. We observe that mSMI consistently outperforms competing methods with little-to-no computational overhead.

==> Figures/NE_k1/Arxiv/NE_k1_maxgrad_rho0.5.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{chocolate2267451}{RGB}{52,138,189}
\definecolor{dimgray85}{RGB}{85,85,85}
\definecolor{gainsboro229}{RGB}{229,229,229}

\begin{axis}[
width=9cm, height=3.5cm,
axis background/.style={fill=gainsboro229},
axis line style={white},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={white},
% xlabel=\textcolor{dimgray85}{\large $n$},
xlabel=\textcolor{dimgray85}{},
xmajorgrids,
xmin=397.164117362141, xmax=62946.2705897083,
xmode=log,
xtick style={color=dimgray85},
xtick={10,100,1000,10000,100000,1000000},
xticklabels={
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\),
  \(\displaystyle {10^{6}}\)
},
y grid style={white},
ylabel=\textcolor{dimgray85}{\large $\msmi$ [nats]},
ymajorgrids,
ymin=0.137318582087755, ymax=0.36,
ytick style={color=dimgray85}
]
\addplot [semithick, chocolate2267451, mark=*, mark size=3, mark options={solid}]
table {%
50000 0.34142941236496
10000 0.342191725969315
5000 0.340315163135529
1000 0.274316489696503
500 0.147074446082115
};
\addplot [semithick, chocolate2267451, dashed]
table {%
50000 0.34142941236496
10000 0.34142941236496
5000 0.34142941236496
1000 0.34142941236496
500 0.34142941236496
100 0.34142941236496
};
\end{axis}

\end{tikzpicture}


==> Figures/auc_d_20_dataset_0.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{dimgray85}{RGB}{85,85,85}
\definecolor{gainsboro229}{RGB}{229,229,229}

\begin{axis}[
width=7cm, height=9cm,
legend style={at={(1,0)}, anchor=south east , fill opacity=0.65, draw opacity=1, text opacity=1, draw=none},
axis background/.style={fill=gainsboro229},
axis line style={white},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={white},
xlabel=\textcolor{dimgray85}{\large n},
xmajorgrids,
xmin=7.94328234724282, xmax=1258.92541179417,
xmode=log,
xtick style={color=dimgray85, font=\large},
xtick={0.1,1,10,100,1000,10000,100000},
xticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\)
},
y grid style={white},
ylabel=\textcolor{dimgray85}{\large ROC AUC},
ymajorgrids,
ymin=0.434615384615385, ymax=1.02692307692308,
ytick style={color=dimgray85, font=\large\textbf}
]
\addplot [semithick, red, legend entries= {$k=2$}]
table {%
10 0.5
32 0.932692307692308
100 1
317 1
1000 1
};
\addplot [semithick, black]
table {%
10 0.461538461538462
32 0.564102564102564
100 0.807692307692308
317 0.961538461538461
1000 0.955128205128205
};
\addplot [semithick, red, dashed]
table {%
10 0.5
32 0.5
100 0.5
317 1
1000 1
};
\addplot [semithick, black, dashed]
table {%
10 0.615384615384615
32 0.891025641025641
100 1
317 1
1000 1
};
\addplot [semithick, red, mark=triangle*, mark size=3, mark options={solid,rotate=180}]
table {%
10 0.5
32 0.5
100 0.5
317 0.791666666666667
1000 1
};
\addplot [semithick, black, mark=triangle*, mark size=3, mark options={solid,rotate=180}]
table {%
10 0.871794871794872
32 1
100 1
317 1
1000 1
};
\addlegendentry{$\asmi, k=2$}
\addlegendentry{$\msmi, k=2$}
\addlegendentry{$\asmi, k=5$}
\addlegendentry{$\msmi, k=5$}
\addlegendentry{$\asmi, k=9$}
\addlegendentry{$\msmi, k=9$}
\end{axis}

\end{tikzpicture}


==> Figures/d20_kk5_dataset_3.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{dimgray85}{RGB}{85,85,85}
\definecolor{gainsboro229}{RGB}{229,229,229}

\begin{axis}[
width=7cm, height=9cm,
legend style={at={(1,0)}, anchor=south east , fill opacity=0.65, draw opacity=1, text opacity=1, draw=none},
axis background/.style={fill=gainsboro229},
axis line style={white},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={white},
xlabel=\textcolor{dimgray85}{n},
xmajorgrids,
xmin=7.94328234724282, xmax=1258.92541179417,
xmode=log,
xtick style={color=dimgray85},
xtick={0.1,1,10,100,1000,10000,100000},
xticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\)
},
y grid style={white},
ylabel=\textcolor{dimgray85}{ROC AUC},
ymajorgrids,
ymin=0.475, ymax=1.025,
ytick style={color=dimgray85}
]
\addplot [semithick, red]
table {%
10 0.5
32 0.865384615384615
100 1
317 1
1000 1
};
\addplot [semithick, black]
table {%
10 0.512820512820513
32 0.705128205128205
100 0.673076923076923
317 0.935897435897436
1000 1
};
\addplot [semithick, red, dashed]
table {%
10 0.5
32 0.5
100 0.5
317 0.5
1000 1
};
\addplot [semithick, black, dashed]
table {%
10 0.762820512820513
32 0.858974358974359
100 1
317 1
1000 1
};
\addplot [semithick, red, mark=triangle*, mark size=3, mark options={solid,rotate=180}]
table {%
10 0.5
32 0.5
100 0.5
317 0.5
1000 0.5
};
\addplot [semithick, black, mark=triangle*, mark size=3, mark options={solid,rotate=180}]
table {%
10 0.775641025641026
32 0.987179487179487
100 0.791666666666667
317 0.583333333333333
1000 0.583333333333333
};
\addlegendentry{$\asmi, k=2$}
\addlegendentry{$\msmi, k=2$}
\addlegendentry{$\asmi, k=5$}
\addlegendentry{$\msmi, k=5$}
\addlegendentry{$\asmi, k=9$}
\addlegendentry{$\msmi, k=9$}
\end{axis}

\end{tikzpicture}

